Gradient-based Discrete Sampling with Automatic Cyclical Scheduling

Discrete distributions, particularly in high-dimensional deep models, are often highly multimodal due to inherent discontinuities. While gradient-based discrete sampling has proven effective, it is susceptible to becoming trapped in local modes due to the gradient information. To tackle this challenge, we propose an automatic cyclical scheduling, designed for efficient and accurate sampling in multimodal discrete distributions. Our method contains three key components: (1) a cyclical step size schedule where large steps discover new modes and small steps exploit each mode; (2) a cyclical balancing schedule, ensuring "balanced" proposals for given step sizes and high efficiency of the Markov chain; and (3) an automatic tuning scheme for adjusting the hyperparameters in the cyclical schedules, allowing adaptability across diverse datasets with minimal tuning. We prove the non-asymptotic convergence and inference guarantee for our method in general discrete distributions. Extensive experiments demonstrate the superiority of our method in sampling complex multimodal discrete distributions.

==> experiments/ebm_learn.tex <==


We also test ACS on deep convolutional EBMs to demonstrate that our method scales to more complex deep neural networks. We use 10 sample steps per iteration on all datasets except Caltech, where we use 30. We include more experimental details along with the generated images in \ref{appndx:sec:exp:ebm_learn}. 

\begin{wraptable}[12]{R}{.6\textwidth}
\centering
\caption{Deep Convolution EBM Log likelihood scores on test data as estimated by AIS. GWG results are taken from \cite{grathwohl2021gwg}. ACS is able to achieve better results than the baselines. }
\begin{tabular}[\textwidth]{lcccl}\toprule
      & GWG\textsuperscript{*}  & DMALA & ACS \\\midrule
Static MNIST & -80.01 & -79.93 & \textbf{-79.76}\\
Dynamic MNIST & -80.51 & -80.13 & \textbf{-79.70} \\
Omniglot & -94.72 & -100.08 & \textbf{-91.32} \\
Caltech & -96.20  & -99.35 & \textbf{-88.34}
\\\bottomrule
\end{tabular}
\label{table:ebm_res}
\end{wraptable}

\paragraph{Results} The results in Table \ref{table:ebm_res} show that our method outperforms DMALA and GWG significantly, even when GWG uses a larger number of sampling steps (40). This can be attributed to our methods ability to explore more modes at a quicker rate, enabling the training process to provide better gradient updates for the model. 

==> experiments/ebm_sample.tex <==
To assess the performance of our sampling method on more complicated energy functions, we adopt a similar experiment set-up to \cite{sun2023anyscale}, where we measure the mixing time of sampling algorithms by how quickly they can achieve better quality samples as measured by the model's unnormalized energy function. 

\paragraph{Results} Figure~\ref{fig:sampling_comp} shows that our method is able to achieve competitive performance on all datasets. On Static/Dynamic MNIST and Omniglot, our method is able to burn in far quicker than other methods. Our method maintains competitive performance on Caltech as well. For more a more detailed discussion on the results, see Appendix \ref{appndx:sec:exp:ebm_sample}.

==> experiments/rbm_sampling.tex <==
We evaluate our method on Restricted Boltzman Machines~(RBMs) trained on various binary datasets. 
RBMs learn the following energy function: 
\begin{align*}
U(\theta) &= \sum_i \text{Softplus}(W \theta + a)_i + b^T \theta
\end{align*}
$\{W, a, b\}$ are parameters for the model, and $\theta \in \{0, 1\}^d$. Following \cite{zhang2022langevinlike, grathwohl2021gwg}, we randomly initialize all samplers and measure the Maximum Mean Divergence (MMD) between the generated samples and those from Block-Gibbs. 
To further test whether ACS can escape local modes, we initialize all samplers to start within the most likely mode of the dataset as measured by the model distribution. 
Block-Gibbs can be regarded as the ground truth for the distribution as it leverages the known structure of the RBM. 

\begin{figure*}[t]
\centering
\includegraphics[width=.9\textwidth]{imgs/rbm_log_mmds_comp_avg.pdf}
\includegraphics[width=.85\textwidth]{imgs/ebm_avg_mixing_times.pdf}

\caption{
Sampling performance of various methods. Top row demonstrates convergence to ground truth on RBMs, bottom row demonstrates mixing speed on deep EBMs. For both distribution types, ACS demonstrates competitive performance with all baselines.
}
\label{fig:sampling_comp}
\end{figure*}

\paragraph{Results} In Figure \ref{fig:sampling_comp}, our method ACS consistently achieves competitive or superior convergence across all datasets, with notable improvements on datasets like caltech. The results also demonstrates that ACS is more robust to mode-specific initialization due to its ability to escape modes. 


